Insights into Security-Related AI-Generated Pull Requests

Recent years have experienced growing contributions of AI coding agents that assist human developers in various software engineering tasks. However, this growing AI-assisted autonomy raises questions about security and trust. In this paper, we analyze more than 33,000 AI-generated pull requests (PRs) and identify 675 security-related submissions made by agentic AIs. Then we examine the security-related PRs with a focus on recurring security weaknesses, review outcomes and latency, commit message quality, and rejection reasons. The results show that security-related AI PRs introduce a small set of recurring weaknesses such as regex inefficiencies, injection flaws, and path traversal. Many flawed contributions are still merged, while rejections often arise from social or process factors such as inactivity or missing test coverage. The commit message quality of AI PRs has a limited effect on acceptance or latency, in contrast to human PRs reported in previous studies. We also extend existing rejection taxonomies by adding categories that are unique to AI-generated security contributions. These findings offer new insights into the strengths and shortcomings of autonomous coding systems in secure software development.

==> sections/method.tex <==


\subsection{RQ1 Methodology}
To investigate the types of security issues introduced by AI PRs, we analyze the code changes using Semgrep~\cite{semgrep} v1.135.0. We select Semgrep for four key reasons.
1. Semgrep provides state-of-the-art static analysis rules covering a wide range of vulnerability classes, enabling consistent detection across projects.
2. Our dataset spans projects implemented in multiple programming languages, and Semgrep offers broad multi-language support (e.g., Java, Python, Go, Rust, JavaScript/TypeScript, PHP, Ruby, Swift), along with package manager and manifest file integration.
3. Semgrep allows fully automated, reproducible scans that can be integrated into a large-scale empirical pipeline.
4. Semgrep has been adopted in several recent software engineering and security studies, demonstrating its effectiveness and acceptance in the research community~\cite{bennett2024semgrep, kluban2024detecting, li2024evaluating, munson2025little}.

For each AI security PR in our dataset, we apply Semgrep scans to both the baseline commit and the PR commit. The baseline commit is the state of the repository before the PR. This setup ensures that we identify only new security issues. 

For each repository we clone the codebase and fetch the PR branch. We then identify the baseline commit with \texttt{git merge-base} against the default branch (for example, \texttt{main} or \texttt{master}). We then run Semgrep on the baseline commit and on the PR commit, saving the outputs in JSON files. We parse the two outputs and compute the set difference to extract the security issues that the PR introduces. This procedure runs for all repositories in the curated set of AI security PRs, producing a structured dataset of newly introduced issues.

\subsection{RQ2 Methodology}

To investigate the factors associated with PR latency and acceptance in AI security PRs, we build on prior empirical studies of PR processes~\cite{zhang2022pull, yu2015wait, dey2020effect, zhang2022pull2}. We consolidate the factors studied in these works, and select those that are both theoretically justified and practically extractable from our dataset.

We extract 24 factors capturing requester experience, PR content, social interactions, project characteristics, and testing signals. The data is collected as of September 15, 2025. Table~\ref{tab:factors} summarizes each factor, its type, and the rationale for inclusion.

\input{tables/factors}

For both PR latency and PR acceptance, we apply the same preprocessing pipeline to ensure data quality, interpretability, and robustness of regression modeling. We handle missing values using \textit{k}-nearest neighbor (KNN) imputation~\cite{zhang2012nearest} with $k=5$.   
We then address infinite values, which occur in derived ratio-based features such as \texttt{requester\_succ\_rate}. Infinite values can destabilize regression coefficients and statistical tests. We therefore replace them with zero, a conservative strategy that prevents invalid computations while keeping the feature in the analysis.  

To reduce the influence of outliers and to improve the linearity assumption of regression models, we apply a logarithmic transformation ($\log(x+1)$) to skewed numeric features, a common strategy in regression modeling~\cite{harrell2015multivariable}. This transformation both compresses the long right tails of distributions (e.g., PR size metrics such as additions and deletions) and ensures that variables with a wide dynamic range are modeled in a scale more suitable for linear regression. Binary variables (e.g., \texttt{first\_pr}, \texttt{friday\_effect}, \texttt{ci\_exists}) remain unchanged since they do not require transformation.  

We mitigate multicollinearity among factors using the \texttt{AutoSpearman} algorithm~\cite{okoye2024correlation}. Multicollinearity inflates variance in coefficient estimates and undermines the interpretability of regression results. \texttt{AutoSpearman} automatically detects pairs of variables with Spearman correlation $\rho \geq 0.7$ and iteratively removes one variable from each pair, retaining the more informative predictor. 


After preprocessing, we conduct two separate regression analyses. 
For \emph{PR latency}, we fit a linear regression model on the log-transformed response time. 
For \emph{PR acceptance}, we fit a logistic regression model that estimates the probability of a PR being merged. 
Both models use the reduced feature set produced by \texttt{AutoSpearman}.

We use evaluation measures that match each model. 
For PR latency, we report the regression coefficients, their significance, the model $R^{2}$, and the adjusted $R^{2}$. 
For PR acceptance, we report odds ratios (OR) with $95\%$ confidence intervals, the associated $p$-values, and the pseudo-$R^{2}$ of Veall–Zimmermann~\cite{veall1996pseudo}. 
At the model level, we also give the chi-square statistic and $p$-value to show whether the factors as a group improve model fit compared to a null model~\cite{harrell2015multivariable}. 


\subsection{RQ3 Methodology}


Prior work shows that messages containing both (\emph{What}) (the description of the change) and (\emph{Why}) (the rationale) provide the highest utility for developers~\cite{tian2022makes}. Tian et al.~\cite{tian2022makes} propose the \emph{C-Good} model, a classifier that identifies whether a commit message contains both elements. Li and Ahmed~\cite{li2023commit} subsequently adopt this model in their study of message quality evolution. Following these works, we employ the same trained model to assess the quality of commit messages in our dataset of AI security PRs.

We extract commit messages for each PR using the GitHub API. To ensure comparability with prior work, we restrict our analysis to English messages. To prepare messages for classification, we replicate the preprocessing steps described by Tian et al.~\cite{tian2022makes}. We normalize commit text by replacing URLs, version numbers, and code snippets with placeholders; remove sign-off information; apply tokenization and part-of-speech tagging; and substitute standardized tokens for reserved placeholders (e.g., \texttt{$url$}, \texttt{$methodName$}). Messages that reduce to empty text are labeled as “empty log message.” This process ensures that our inputs align with the data used to train the original model.

Tian et al.~\cite{tian2022makes} frame commit message quality as a binary classification problem. The annotated dataset contains four labels: messages that include both Why and What (label 0), messages that include neither (label 1), messages that omit What (label 2), and messages that omit Why (label 3). For modeling, labels 1–3 collapse into a single bad category, while label 0 represents the good category. This setup yields a binary classification task, where label 0 indicates a commit message that contains both Why and What, and label 1 denotes any message that omits one or both elements.

Tian et al.~\cite{tian2022makes} report that their \emph{C-Good} model, a BERT encoder with a BiLSTM classification head, achieves the highest performance among tested baselines, with an F1-score exceeding 0.80. We retrain the C-Good model on the original dataset using the prescribed preprocessing pipeline. We then apply the trained model to the commit messages from our AI security PR dataset.

For inference, we preprocess all commit messages using the same pipeline to ensure input compatibility. The preprocessed messages pass through the trained C-Good model, which outputs for each commit a binary label (good or bad) together with a confidence score derived from the softmax probability of the predicted class.


\subsection{RQ4 Methodology}
\label{sec:rq4_method}

To address this question, we investigate the reasons why AI-generated security PRs are rejected by maintainers. Following prior work by Watanabe et al.~\cite{watanabe2025use}, we define \textit{rejected PRs} as those that are closed without being merged. Our analysis focuses on rejection reasons, which we derive through a combination of established classification schemes and inductive coding.

We adopt the rejection taxonomy proposed by Pantiuchina et al.~\cite{pantiuchina2021developers}, as extended by Watanabe et al.~\cite{watanabe2025use}. This framework has been validated in empirical studies of code review and captures both process-related and technical reasons for rejection. Specifically, we employ the 14 categories reported by Watanabe et al., which span a wide range of rejection patterns independent of PR type.

During our inspection, we encounter rejection reasons that do not fit the above categories. To capture these, we apply an \textit{open card-sorting technique}: both annotators independently group the new comments into candidate categories, then reconcile differences through discussion. This process yields two additional rejection reasons that extend the existing framework to better account for AI-generated security PRs.

Two independent authors manually inspect the maintainer comments associated with rejected PRs. Each annotator assigns one rejection category per PR. The initial agreement is 74.5\%, corresponding to a Cohen’s $\kappa$ of 0.57, which indicates \textit{moderate agreement}~\cite{landis1977measurement}. Disagreements are resolved through discussion until consensus is reached.











==> tables/issue_summary.tex <==
\begin{table*}[h]
\centering
\caption{Semgrep issues by AI PR category and PR outcome. Top 3 CWEs are listed with counts.}
\label{tab:ai_pr_outcome}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|r|r|r|l|}
\hline
\textbf{AI PR Category} & \textbf{PR Outcome} & \textbf{Total PRs} & \textbf{PRs with $\geq$1 Issue} & \textbf{\% with Issue} & \textbf{Top 3 CWEs (count)} \\
\hline \hline
& Accepted & 22  & 5  & 22.7\% & CWE-532 (6), CWE-134 (5), CWE-918 (3) \\\cline{2-6}
   Claude Code             & Open     & 2   & 0  & 0.0\%  & -- \\\cline{2-6}
              & Rejected & 9   & 1  & 11.1\% & CWE-78 (2) \\\hline
       & Accepted & 110 & 13 & 11.8\% & CWE-22 (12), CWE-79 (9), CWE-78 (5) \\\cline{2-6}
     Copilot         & Open     & 69  & 15 & 21.7\% & CWE-79 (14), CWE-22 (9), CWE-639 (8) \\\cline{2-6}
              & Rejected & 103 & 15 & 14.6\% & CWE-1333 (289), CWE-78 (92), CWE-798 (40) \\\hline
        & Accepted & 27  & 3  & 11.1\% & CWE-134 (4), CWE-1333 (3), CWE-327 (1) \\\cline{2-6}
       Cursor      & Open     & 12  & 5  & 41.7\% & CWE-134 (19), CWE-295 (5), CWE-319 (1) \\\cline{2-6}
              & Rejected & 15  & 3  & 20.0\% & CWE-319 (3), CWE-134 (2), CWE-798 (1) \\\hline
         & Accepted & 74  & 15 & 20.3\% & CWE-22 (16), CWE-79 (9), CWE-1333 (7) \\\cline{2-6}
       Devin       & Open     & 14  & 3  & 21.4\% & CWE-78 (3), CWE-134 (2), CWE-116 (1) \\\cline{2-6}
              & Rejected & 76  & 10 & 13.2\% & CWE-134 (35), CWE-22 (13), CWE-1333 (6) \\\hline
 & Accepted & 121 & 15 & 12.4\% & CWE-22 (29), CWE-470 (14), CWE-95 (8) \\\cline{2-6}
       OpenAI Codex       & Open     & 5   & 1  & 20.0\% & CWE-79 (2), CWE-522 (1) \\\cline{2-6}
              & Rejected & 16  & 0  & 0.0\%  & -- \\\hline
\end{tabular}
}
\end{table*}



